Domain Game: Disentangle Anatomical Feature for Single Domain Generalized Segmentation

Single domain generalization aims to address the challenge of out-of-distribution generalization problem with only one source domain available. Feature distanglement is a classic solution to this purpose, where the extracted task-related feature is presumed to be resilient to domain shift. However, the absence of references from other domains in a single-domain scenario poses significant uncertainty in feature disentanglement (ill-posedness). In this paper, we propose a new framework, named \textit{Domain Game}, to perform better feature distangling for medical image segmentation, based on the observation that diagnostic relevant features are more sensitive to geometric transformations, whilist domain-specific features probably will remain invariant to such operations. In domain game, a set of randomly transformed images derived from a singular source image is strategically encoded into two separate feature sets to represent diagnostic features and domain-specific features, respectively, and we apply forces to pull or repel them in the feature space, accordingly. Results from cross-site test domain evaluation showcase approximately an ~11.8% performance boost in prostate segmentation and around ~10.5% in brain tumor segmentation compared to the second-best method.

==> TODO.tex <==
5. The choice of the title "Domain Game" seems unrelated to combinatorial games, and the connection between the proposed method and combinatorial games is not adequately clarified. Although the authors briefly discussed this analogy in the subsection "Analogy to Combinatorial Game," further clarification is needed. If the authors wish to establish an equivalence between the proposed method and a combinatorial game, it is recommended to provide theoretical or mathematical proof. (#2)  
7. The method involves maximizing utilities, but it is not apparent why formulating the optimization process as a minimax strategy is necessary. Maximizing the Dice metric and PSNR is equivalent to minimizing the dice loss and MSE loss, respectively. Further clarification on the motivation for employing a minimax strategy would be beneficial. (#2)   9. The concept of a combinatorial game seems to be reminiscent of existing techniques in contrastive learning.(#3)



typos: "endervor" in page to should be "endeavor"


5. In Table 3, the column "Avg. of Both Tasks" seems to provide minimal information and may be unnecessary. (#3)


4. Please update the reference to BayeSeg to the latest version. (#3)



6. The rationale behind incorporating a Lasso loss for feature space shrinkage requires further theoretical elaboration. Can the authors provide a more in-depth explanation? Additionally, it would be helpful to explore whether alternative loss functions can be used as replacement (#2)	

"Lasso is a common and widely applied way for space shrinkage, we appreciate the suggestion as there are many possible way of shrinkage choice, and would benefit if can be tested, we actually try out RMS, and it tend to make all the feature value smaller, which is not equal to shrinkage (to scatter the feature in feature vector, make them zero): [1] Regression Shrinkage and Selection via the Lasso

作者：R TIBSHIRANI · 被引用次数：58856 — As pointed out by Jerome Friedma"
7. While the authors introduce data-based methods and highlight their vulnerability to substantial domain shifts, a comparison with "Causality-inspired single-source domain generalization for medical image segmentation" is missing from the experimental evaluation. It is recommended to include such a comparison in the experiments.(#2)	比较 Casulaity, 我们appreciate 他的贡献, 




==> imgs/ID.tex <==
\begin{wrapfigure}{r}{0.42\textwidth}
\begin{center}
\vspace{-1.3cm}
  \includegraphics[width=0.44\textwidth ]{id.png}
\end{center}
\vspace{-7mm}  % -4
\caption{\small Hi.}
\label{fig:ID}
\vspace{-3em}
\end{wrapfigure}



% \begin{wrapfigure}{r}{0.495\textwidth}
% \begin{center}
% \begin{figure}
%     \centering
%     \includegraphics[width=1.0\linewidth]{id.png}
% \end{figure}
% \vspace{-4mm}  
% \end{center}
%  \caption{Enter Caption}
% \label{fig:id}
% \vspace{-3em}
% \end{wrapfigure}



% \begin{figure}
%     \centering
%     \includegraphics[width=0.5\linewidth]{图片.png}
%     \caption{Enter Caption}
%     \label{fig:enter-label}
% \end{figure}

==> sections/math.tex <==

\begin{theorem}
This is a sample theorem. The run-in heading is set in bold, while
the following text appears in italics. Definitions, lemmas,
propositions, and corollaries are styled the same way.
\end{theorem}



\begin{proof}
Proofs, examples, and remarks have the initial word in italics,
while the following text appears in normal font.
\end{proof}


% articles~\cite{ref_article1}, an LNCS chapter~\cite{ref_lncs1}, a
% book~\cite{ref_book1}, proceedings without editors~\cite{ref_proc1},

For citations of references, we prefer the use of square brackets
and consecutive numbers. Citations using labels or the author/year
convention are also acceptable. The following bibliography provides
a sample reference list with entries for journal

and a homepage~\cite{ref_url1}. Multiple citations are grouped
\cite{ref_article1,ref_lncs1,ref_book1},
\cite{ref_article1,ref_book1,ref_proc1,ref_url1}.

\begin{credits}
\subsubsection{\ackname} A bold run-in heading in small font size at the end of the paper is
used for general acknowledgments, for example: This study was funded
by X (grant number Y).

\subsubsection{\discintname}
It is now necessary to declare any competing interests or to specifically
state that the authors have no competing interests. Please place the
statement with a bold run-in heading in small font size beneath the
(optional) acknowledgments\footnote{If EquinOCS, our proceedings submission
system, is used, then the disclaimer can be provided directly in the system.},
for example: The authors have no competing interests to declare that are
relevant to the content of this article. Or: Author A has received research
grants from Company W. Author B has received a speaker honorarium from
Company X and owns stock in Company Y. Author C is a member of committee Z.
\end{credits}
